Password-authenticated Decentralized Identities

Password-authenticated identities, where users establish username-password pairs with individual servers and use them later on for authentication, is the most widespread user authentication method over the Internet. Although they are simple, user-friendly, and broadly adopted, they offer insecure authentication and position server operators as trusted parties, giving them full control over users' identities. To mitigate these limitations, many identity systems have embraced public-key cryptography and the concept of decentralization. All these systems, however, require users to create and manage public-private keypairs. Unfortunately, users usually do not have the required knowledge and resources to properly handle their cryptographic secrets, which arguably contributed to failures of many end-user-focused public-key infrastructures (PKIs). In fact, as for today, no end-user PKI, able to authenticate users to web servers, has a significant adoption rate. In this paper, we propose Password-authenticated Decentralized Identities (PDIDs), an identity and authentication framework where users can register their self-sovereign username-password pairs and use them as universal credentials. Our system provides global namespace, human-meaningful usernames, and resilience against username collision attacks. A user's identity can be used to authenticate the user to any server without revealing that server anything about the password, such that no offline dictionary attacks are possible against the password. We analyze PDIDs and implement it using existing infrastructures and tools. We report on our implementation and evaluation.

==> sec/disc.tex <==
\section{Discussion on \name Management}
\label{sec:overview:mgmt}
\names, being password-authenticated identities, share multiple similarities
with password management. However, the decentralization
brings to \names some inherent and interesting limitations which have not been
investigated in the context of password-based credentials (up to our best
knowledge, \names is the first system of this class).  These limitations are
generic and are mainly due to a lack of out-of-band mechanisms  which in
traditional authentication systems allow users to recover or change their
passwords (like customer support or e-mail recovery). With \names, all
password-related rules and policies have to be encoded in the GPM's code, which
introduces multiple trade-offs.

For instance, password updates can be implemented with \names as sketched
here. For a new password $pwd'$, the user could generate its new metadata
$m'=\langle k_s',p_s',P_s',P_u',c'\rangle,$
and send it together with its username and the old password in an encrypted
transaction: % \footnote{If desired, sending the old password could be avoided.
% The user and the GPM could run the authentication process instead, after which
% the user would send a termination request encrypted with the computed session
% key.  That would, however, impose more complexity in the GPM's code and,
% potentially, require strong randomness from the GPM.  (In fact, such a technique
% could be used for the \name registration too.)}
$\PEnc{pk_b}{U, pwd, m'}.$
That would trigger a GPM's password update method, which would restore the `old'
metadata and verify if the sent password matches it by computing and checking
the following:
$k\gets\Fk{k_s}{pwd};\langle p_u, P_u, P_s\rangle\overset{?}{=}\ADec{k}{c};g^{p_u}\overset{?}{=}P_u.$
If so, the method would update the GPM's state by the new metadata as
$users[U]\gets m'.$
(Additionally, the authentication method \texttt{AuthPDID()} would need to ensure
that the authentication is conducted using the current password.)

Such a password update procedure; however, would introduce a risk that in the case of a password
compromise, the adversary could hijack the identity  permanently (by
simply changing the password).  Therefore, password-authenticated decentralized
identities may require alternative management practices.  For instance, a
mechanism of identity termination, when a user wishes to permanently invalidate
its (e.g., compromised) identity, seems to be more appropriate in some
scenarios.  Other mechanisms easily implementable with \names  include
establishing a secondary password for password recovery/update.  All these
mechanisms could be implemented in a similar way as the password update
mechanism. Similarly, \names could be integrated with some second-factor
authenticators, that could be established together with user identities.
We leave details of these constructions and their analysis as future
work; however.

